Curvature Aligned Simplex Gradient: Principled Sample Set Construction For Numerical Differentiation

The simplex gradient, a popular numerical differentiation method due to its flexibility, lacks a principled method by which to construct the sample set, specifically the location of function evaluations. Such evaluations, especially from real-world systems, are often noisy and expensive to obtain, making it essential that each evaluation is carefully chosen to reduce cost and increase accuracy. This paper introduces the curvature aligned simplex gradient (CASG), which provably selects the optimal sample set under a mean squared error objective. As CASG requires function-dependent information often not available in practice, we additionally introduce a framework which exploits a history of function evaluations often present in practical applications. Our numerical results, focusing on applications in sensitivity analysis and derivative free optimization, show that our methodology significantly outperforms or matches the performance of the benchmark gradient estimator given by forward differences (FD) which is given exact function-dependent information that is not available in practice. Furthermore, our methodology is comparable to the performance of central differences (CD) that requires twice the number of function evaluations.

==> figs/Quadratic_eCASG/sig_0.1_num_1000_32d_Error.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange}{RGB}{255,140,0}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{slategray}{RGB}{112,128,144}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=lightgray204
},
log basis x={10},
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={k},
xmajorgrids,
xmin=3.98107170553497e-05, xmax=25118.8643150958,
xmode=log,
xtick style={color=black},
y grid style={darkgray176},
ylabel={MSE},
ymajorgrids,
ymin=0.00540055449998526, ymax=4272.67155457127,
ymode=log,
ytick style={color=black}
]
\path [draw=slategray, very thick]
(axis cs:0.0001,2.10776798219624)
--(axis cs:0.0001,6.4107783676559);

\path [draw=slategray, very thick]
(axis cs:0.000215443469003188,2.11720034793963)
--(axis cs:0.000215443469003188,6.42022420850028);

\path [draw=slategray, very thick]
(axis cs:0.000464158883361278,2.11815173937331)
--(axis cs:0.000464158883361278,6.42120463115893);

\path [draw=slategray, very thick]
(axis cs:0.001,2.11655648559142)
--(axis cs:0.001,6.41919349992927);

\path [draw=slategray, very thick]
(axis cs:0.00215443469003188,2.11599422160635)
--(axis cs:0.00215443469003188,6.41880879886977);

\path [draw=slategray, very thick]
(axis cs:0.00464158883361277,2.11904250592116)
--(axis cs:0.00464158883361277,6.42223963091116);

\path [draw=slategray, very thick]
(axis cs:0.01,2.11261910819059)
--(axis cs:0.01,6.44199262969641);

\path [draw=slategray, very thick]
(axis cs:0.0215443469003188,2.10949817668911)
--(axis cs:0.0215443469003188,6.43928142491498);

\path [draw=slategray, very thick]
(axis cs:0.0464158883361277,2.10918230019451)
--(axis cs:0.0464158883361277,6.43883265577852);

\path [draw=slategray, very thick]
(axis cs:0.1,2.11378029196098)
--(axis cs:0.1,6.44792795216787);

\path [draw=slategray, very thick]
(axis cs:0.215443469003188,2.12716983570316)
--(axis cs:0.215443469003188,6.46663293321699);

\path [draw=slategray, very thick]
(axis cs:0.464158883361277,2.13954145797152)
--(axis cs:0.464158883361277,6.51257824992227);

\path [draw=slategray, very thick]
(axis cs:1,2.16840740037035)
--(axis cs:1,6.62919932046866);

\path [draw=slategray, very thick]
(axis cs:2.15443469003188,2.19885996036197)
--(axis cs:2.15443469003188,6.88550771204933);

\path [draw=slategray, very thick]
(axis cs:4.64158883361277,2.35074679299626)
--(axis cs:4.64158883361277,7.33857772357037);

\path [draw=slategray, very thick]
(axis cs:10,2.54489722830905)
--(axis cs:10,8.51060683180087);

\path [draw=slategray, very thick]
(axis cs:21.5443469003188,3.07934044997555)
--(axis cs:21.5443469003188,11.1619730700301);

\path [draw=slategray, very thick]
(axis cs:46.4158883361277,3.88132547341951)
--(axis cs:46.4158883361277,17.0372133967907);

\path [draw=slategray, very thick]
(axis cs:100,5.23978556551105)
--(axis cs:100,29.1799113152706);

\path [draw=slategray, very thick]
(axis cs:215.443469003188,8.39802011710026)
--(axis cs:215.443469003188,55.5069870226113);

\path [draw=slategray, very thick]
(axis cs:464.158883361277,14.9690746615304)
--(axis cs:464.158883361277,112.449055130344);

\path [draw=slategray, very thick]
(axis cs:1000,28.8673310653799)
--(axis cs:1000,235.726440484475);

\path [draw=slategray, very thick]
(axis cs:2154.43469003188,59.1006647729909)
--(axis cs:2154.43469003188,500.802739820119);

\path [draw=slategray, very thick]
(axis cs:4641.58883361277,126.529109224481)
--(axis cs:4641.58883361277,1070.08011520697);

\path [draw=slategray, very thick]
(axis cs:10000,268.877408280276)
--(axis cs:10000,2304.60621917221);

\path [draw=darkorange, very thick]
(axis cs:0.0001,0.0100124678129555)
--(axis cs:0.0001,0.0117807762288068);

\path [draw=darkorange, very thick]
(axis cs:0.000215443469003188,0.0146959556312098)
--(axis cs:0.000215443469003188,0.0172859123282661);

\path [draw=darkorange, very thick]
(axis cs:0.000464158883361278,0.0215567310230058)
--(axis cs:0.000464158883361278,0.025373912954204);

\path [draw=darkorange, very thick]
(axis cs:0.001,0.0316334353800312)
--(axis cs:0.001,0.0372744883096043);

\path [draw=darkorange, very thick]
(axis cs:0.00215443469003188,0.0464209761333135)
--(axis cs:0.00215443469003188,0.0546571971590382);

\path [draw=darkorange, very thick]
(axis cs:0.00464158883361277,0.0680041318572159)
--(axis cs:0.00464158883361277,0.0802416571817834);

\path [draw=darkorange, very thick]
(axis cs:0.01,0.0997269422240541)
--(axis cs:0.01,0.117756800102704);

\path [draw=darkorange, very thick]
(axis cs:0.0215443469003188,0.146359671807978)
--(axis cs:0.0215443469003188,0.172945596225756);

\path [draw=darkorange, very thick]
(axis cs:0.0464158883361277,0.214809813955036)
--(axis cs:0.0464158883361277,0.254524544754158);

\path [draw=darkorange, very thick]
(axis cs:0.1,0.314535599624728)
--(axis cs:0.1,0.376099619792131);

\path [draw=darkorange, very thick]
(axis cs:0.215443469003188,0.458976837203496)
--(axis cs:0.215443469003188,0.560395612741658);

\path [draw=darkorange, very thick]
(axis cs:0.464158883361277,0.664188624545397)
--(axis cs:0.464158883361277,0.837780403223117);

\path [draw=darkorange, very thick]
(axis cs:1,0.950626153452963)
--(axis cs:1,1.26969689713664);

\path [draw=darkorange, very thick]
(axis cs:2.15443469003188,0.969090820218)
--(axis cs:2.15443469003188,1.28832668314709);

\path [draw=darkorange, very thick]
(axis cs:4.64158883361277,0.993492089791496)
--(axis cs:4.64158883361277,1.31262579763313);

\path [draw=darkorange, very thick]
(axis cs:10,1.02237362273299)
--(axis cs:10,1.34938075546615);

\path [draw=darkorange, very thick]
(axis cs:21.5443469003188,1.06422095706302)
--(axis cs:21.5443469003188,1.40369310181309);

\path [draw=darkorange, very thick]
(axis cs:46.4158883361277,1.12534607751684)
--(axis cs:46.4158883361277,1.48389521405121);

\path [draw=darkorange, very thick]
(axis cs:100,1.21207090224717)
--(axis cs:100,1.59840192238638);

\path [draw=darkorange, very thick]
(axis cs:215.443469003188,1.31808378002272)
--(axis cs:215.443469003188,1.76736364036072);

\path [draw=darkorange, very thick]
(axis cs:464.158883361277,1.48800457360283)
--(axis cs:464.158883361277,2.02776063706335);

\path [draw=darkorange, very thick]
(axis cs:1000,1.70832149638228)
--(axis cs:1000,2.40664046762865);

\path [draw=darkorange, very thick]
(axis cs:2154.43469003188,2.02786764358689)
--(axis cs:2154.43469003188,2.99429215475097);

\path [draw=darkorange, very thick]
(axis cs:4641.58883361277,2.47626723285838)
--(axis cs:4641.58883361277,3.88120824897139);

\path [draw=darkorange, very thick]
(axis cs:10000,3.12249019365124)
--(axis cs:10000,5.26065034853419);

\addplot [ultra thick, darkorange]
table {%
0.0001 0.0109601739264751
0.000215443469003188 0.0160873671488317
0.000464158883361278 0.0236131265515431
0.001 0.0346596487083128
0.00215443469003188 0.0508744152082203
0.00464158883361277 0.0746766171509219
0.01 0.10962036117877
0.0215443469003188 0.160932529758156
0.0464158883361277 0.236317192177052
0.1 0.347183089884673
0.215443469003188 0.510590112508091
0.464158883361277 0.752544100679252
1 1.11409699811647
2.15443469003188 1.13038703574788
4.64158883361277 1.1543093247003
10 1.18944638655005
21.5443469003188 1.24106796892895
46.4158883361277 1.31692877387926
100 1.42844247207783
215.443469003188 1.5924049687434
464.158883361277 1.83351587286749
1000 2.18806051250595
2154.43469003188 2.70929063367219
4641.58883361277 3.47531101182474
10000 4.60067059468029
};
\addlegendentry{CASG}
\addplot [ultra thick, slategray, dashed]
table {%
0.0001 4.65001499999998
0.000215443469003188 4.65003231652039
0.000464158883361278 4.65006962383254
0.001 4.65015000000004
0.00215443469003188 4.65032316520348
0.00464158883361277 4.65069623832502
0.01 4.65150000000004
0.0215443469003188 4.65323165203503
0.0464158883361277 4.65696238325045
0.1 4.66499999999998
0.215443469003188 4.68231652035051
0.464158883361277 4.71962383250423
1 4.80000000000004
2.15443469003188 4.97316520350477
4.64158883361277 5.34623832504196
10 6.15000000000003
21.5443469003188 7.88165203504786
46.4158883361277 11.6123832504195
100 19.6500000000002
215.443469003188 36.9665203504733
464.158883361277 74.2738325041807
1000 154.650000000046
2154.43469003188 327.815203504406
4641.58883361277 700.888325042176
10000 1504.65000001355
};
\addlegendentry{FD}

\end{axis}

\end{tikzpicture}


==> figs/Quadratic_eCASG/sig_0.1_num_1000_32d_S_scale.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange}{RGB}{255,140,0}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{slategray}{RGB}{112,128,144}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
log basis x={10},
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={k},
xmajorgrids,
xmin=3.98107170553497e-05, xmax=25118.8643150958,
xmode=log,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Radius},
ymajorgrids,
ymin=0.444232827975337, ymax=1053.98948130671,
ymode=log,
ytick style={color=black}
]

\addplot [ultra thick, darkorange]
table {%
0.0001 740.315649436376
0.000215443469003188 416.33617288287
0.000464158883361278 234.154640358874
0.001 131.713113477651
0.00215443469003188 74.1140869469334
0.00464158883361277 41.7335273585927
0.01 23.5363320947428
0.0215443469003188 13.317291715057
0.0464158883361277 7.58710382544592
0.1 4.38329330870497
0.215443469003188 2.60096094813883
0.464158883361277 1.61572056341395
1 1.07187337372826
2.15443469003188 1.07268061323789
4.64158883361277 1.07597895686481
10 1.08225987376237
21.5443469003188 1.09244727070029
46.4158883361277 1.10801634019381
100 1.13116121910343
215.443469003188 1.16499567995537
464.158883361277 1.21374661310052
1000 1.28287912113888
2154.43469003188 1.37910419656063
4641.58883361277 1.51028261589319
10000 1.68531803959694
};
\addlegendentry{CASG}
\addplot [ultra thick, slategray, dashed]
table {%
0.0001 63.2455532033676
0.000215443469003188 43.0886938006377
0.000464158883361278 29.3559853524414
0.001 20
0.00215443469003188 13.6258413811592
0.00464158883361277 9.28317766722556
0.01 6.32455532033676
0.0215443469003188 4.30886938006377
0.0464158883361277 2.93559853524414
0.1 2
0.215443469003188 1.36258413811592
0.464158883361277 0.928317766722556
1 0.632455532033676
2.15443469003188 0.632455532033676
4.64158883361277 0.632455532033676
10 0.632455532033676
21.5443469003188 0.632455532033676
46.4158883361277 0.632455532033676
100 0.632455532033676
215.443469003188 0.632455532033676
464.158883361277 0.632455532033676
1000 0.632455532033676
2154.43469003188 0.632455532033676
4641.58883361277 0.632455532033676
10000 0.632455532033676
};
\addlegendentry{FD}
\end{axis}

\end{tikzpicture}

